Bayesian Online Natural Gradient (BONG)

We propose a novel approach to sequential Bayesian inference based on variational Bayes (VB). The key insight is that, in the online setting, we do not need to add the KL term to regularize to the prior (which comes from the posterior at the previous timestep); instead we can optimize just the expected log-likelihood, performing a single step of natural gradient descent starting at the prior predictive. We prove this method recovers exact Bayesian inference if the model is conjugate. We also show how to compute an efficient deterministic approximation to the VB objective, as well as our simplified objective, when the variational distribution is Gaussian or a sub-family, including the case of a diagonal plus low-rank precision matrix. We show empirically that our method outperforms other online VB methods in the non-conjugate setting, such as online learning for neural networks, especially when controlling for computational costs.

==> abstract.tex <==
\begin{abstract}
  We propose a novel approach to  sequential Bayesian inference based on variational Bayes (VB).
  The key insight is that,
  in the online setting,
  we do not need to add the KL term to regularize to the prior (which comes from the posterior at the previous timestep);
  instead we can optimize just the expected log-likelihood,
  performing a single step of natural gradient descent
  starting at the prior predictive.
  We prove this method
 recovers exact Bayesian inference 
  if the model is conjugate.
 %
\rev{We also  show how to compute an
 efficient deterministic 
 approximation to the VB objective,
  as well as our simplified objective,
 when the variational distribution is
 Gaussian or a sub-family, including the case of
 a diagonal plus low-rank
precision matrix.}
%
We show empirically that our
method outperforms other online VB methods
  in the  non-conjugate setting,
  such as online learning for neural networks,
  especially when controlling for computational costs.
\end{abstract}

==> algo_overview.tex <==
\subsection{Overall space of methods}
\label{sec:method-space}

\input{online-ND sections/table-algo}

\eat{
\Cref{tab:methods} lists the space of methods we consider defined by five binary contrasts: 
update via NGD vs.\ GD, 
loss defined by $\expect{\rm NLL}$ vs.\ VI, integration via MC vs.\ linearizing,
FC vs.\ DLR family,
and natural vs.\ source parameterization.
}

Crossing the four algorithms in \cref{tab:space}, 
\rev{the four methods of approximating the Hessian in \cref{tab:hessian}, and the five variational families yields 80 algorithms. \Cref{tab:methods} shows the 36 based on the three tractable Hessian approximations and the three variational families that use natural parameters.}
% \kpm{
% the three tractable
% methods of approximating the Hessian
% in \cref{tab:hessian},
% and  the 3 
% variational families  yields 36 algorithms,
% shown in \cref{tab:methods}.
% }
% which can be categorized based on the following factors:
% update via NGD vs.\ GD;
% loss defined by $\expect{\rm NLL}$ vs.\ VI;
% predictive distribution approximated with MC vs.\ linearization;
% true Hessian vs.\ empirical Fisher;
% full, diagonal, or DLR form for the covariance/precision; 
% and natural vs.\ moment (or DLR) parameters.
\eat{
\Cref{tab:methods} lists 40 of the methods
(focusing on the \efmc and \hesslin
Hessian approximations that we use in our experiments),
and states their time complexity, in terms of
$\nparam$, the dimensionality  of the parameter space;
$\nsample$, the number of MC samples (not relevant for the linearized variants);
$\niter$, the number of iterations per time step
(we fix $\niter=1$ for \bong and \bog variants);
$\rank$, the rank of the DLR approximation
(not relevant for full or diagonal covariance); and
$\nout$, the size of the output vector $\vy_t$
(relevant only for the \hesslin variants).
}
Update equations for all the algorithms are derived in \cref{sec:derivations}.
Pseudocode is given in \cref{sec:pseudocode}.


==> packages.tex <==

\newcommand{\myeat}[1]{}
%http://www.stackprinter.com/export?service=tex.stackexchange&question=59702&printer=false&linktohome=true

%\usepackage[framemethod=TikZ]{mdframed}

% https://tex.stackexchange.com/questions/99049/latex-error-option-clash-for-package-xcolor-even-if-i-put-listings-before
%https://en.wikibooks.org/wiki/LaTeX/Colors
\usepackage[usenames,dvipsnames]{xcolor}
%\usepackage[usenames]{color}

%\usepackage{float}
\usepackage{longtable}

\usepackage[toc,page]{appendix}

%\usepackage{tocloft}
%\advance\cftchapnumwidth 1cm
%https://tex.stackexchange.com/questions/436063/spacing-between-number-and-text-in-toc
%\advance\cftsecnumwidth 0.5em\relax


% https://mirror.las.iastate.edu/tex-archive/macros/latex/contrib/mathalpha/doc/mathalpha-doc.pdf
\usepackage{bm}
\usepackage{frcursive} 
\usepackage{xfrac}
\usepackage{mathrsfs}

\usepackage{fancyvrb} % https://tex.stackexchange.com/questions/122195/how-to-center-verbatim
\usepackage{xspace}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}

%https://tex.stackexchange.com/questions/58098/what-are-all-the-font-styles-i-can-use-in-math-mode
\usepackage[mathscr]{euscript}

\mathchardef\mhyphen="2D % Define a "math hyphen"
\mathchardef\mdash="2D % Define a "math hyphen"

%\usepackage{undertilde}
\usepackage{accents}


\usepackage[font={small,it}]{caption}
%\usepackage{subfigure}
\usepackage{subcaption} 
\usepackage{subfig}
%\usepackage{caption}
%\usepackage[font={small,it}]{subcaption} % https://en.wikibooks.org/wiki/LaTeX/Floats,_Figures_and_Captions#Subfloats

%https://tex.stackexchange.com/questions/283324/different-font-sizes-for-figure-and-subfigure-captions/283327
%\captionsetup{font={footnotesize,it}}
%\captionsetup[sub]{font={footnotesize,it}}

%\usepackage[font={small,it}]{caption}
%\usepackage[font={footnotesize,it}]{caption}

\usepackage{url}
\usepackage{cancel} % \cancel for strikethrough
\usepackage{multirow}
\usepackage{multicol}




\usepackage{verbatim}
%\usepackage{comment} %http://www.ctan.org/tex-archive/macros/latex/contrib/comment/

% From https://media.nips.cc/Conferences/NIPS2017/Styles/nips_2017.tex
% https://tex.stackexchange.com/questions/406179/how-to-type-the-letter-%C5%81

\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% https://tex.stackexchange.com/questions/392208/command-k-unavailable-in-encoding-ot1-error-takes-me-to-line-which-doesnt-eve

%http://mirrors.ibiblio.org/CTAN/macros/latex/base/utf8ienc.pdf
\usepackage[utf8]{inputenc}
%\DeclareUnicodeCharacter{2010}{-}% support older LaTeX versions
%\DeclareUnicodeCharacter{2212}{-}% support older LaTeX versions
%\DeclareUnicodeCharacter{301}{-}% support older LaTeX versions
%\DeclareUnicodeCharacter{00B4}{\textasciiacute}
\DeclareUnicodeCharacter{00B4}{'}


\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography



%https://tex.stackexchange.com/questions/36660/only-authors-initials-in-bibtex-natbib-using-named-style

%http://mirrors.ibiblio.org/CTAN/macros/latex/exptl/biblatex/doc/biblatex.pdf
%  bibstyle=authortitle,
\usepackage[
  style=alphabetic,
  citestyle=alphabetic,
  natbib=true,
  backend=bibtex,
  maxcitenames=3,  mincitenames=1,
  maxbibnames=10,  minbibnames=1,
  firstinits=true,
  backref=false, 
  hyperref=true,
  doi=false,  isbn=false,  url=false,
  arxiv=abs
]{biblatex}

%https://tex.stackexchange.com/questions/36307/formatting-back-references-in-bibliography
\DefineBibliographyStrings{english}{%
  backrefpage = {page},% originally "cited on page"
  backrefpages = {pages},% originally "cited on pages"
}

\usepackage{xpatch}

\usepackage{booktabs}
\usepackage{comment}

\usepackage{paralist} % compactenunm, compactitem

\usepackage{tikz}
\usetikzlibrary{fit,arrows,calc,positioning,shadows.blur}

% https://www.overleaf.com/learn/how-to/Cross_referencing_with_the_xr_package_in_Overleaf
%https://tex.stackexchange.com/questions/14364/cross-referencing-between-different-files?noredirect=1&lq=1
%https://texfaq.org/FAQ-extref
\usepackage{xr}
%\usepackage{xr-hyper}
%\usepackage{zref-xr,zref-user}

%\externaldocument{app}


% From 	Mykel Kochenderfer 
\usepackage{mathtools}
\DeclarePairedDelimiter{\paren}{\lparen}{\rparen}
\DeclarePairedDelimiter{\brock}{\lbrack}{\rbrack}

\usepackage{enumitem}


%\usepackage{algorithm}
%\usepackage{algpseudocode}

% https://jdhao.github.io/2019/09/21/latex_algorithm_pseudo_code/

\usepackage[ruled,vlined,linesnumbered,algochapter]{algorithm2e}
%\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
%\usepackage[noend]{algpseudocode}
%\usepackage{algorithmic}
\DontPrintSemicolon
\newcommand{\dontprintsemicolon}{}
% https://tex.stackexchange.com/questions/192435/adding-a-blank-line-in-algorithm2e

\usepackage{mdframed}
\usepackage{multicol}
\usepackage{rotating}
\usepackage{setspace}



\usepackage{blkarray}



%https://www.tug.org/FontCatalogue/newpx/
%https://wiki.carleton.edu/download/attachments/20155418/fontguide.pdf?version=1&modificationDate=1388599695000&api=v2
%\usepackage{newpxmath,newpxtext}

% https://tex.stackexchange.com/questions/514149/three-column-full-page-index-in-tufte-booktwoside-symmetric
%\usepackage[makeindex]{imakeidx}
\usepackage{imakeidx}
\usepackage[columns=3]{idxlayout}

% Hyperref needs to be last package
%https://tex.stackexchange.com/questions/326950/hyperref-conflicts-with-footnotea
%\usepackage[pagebackref=true,colorlinks=true,pdftex]{hyperref} % incompatible
%\usepackage[backref=true,colorlinks=true,pdftex]{hyperref} % incompatible

% https://tex.stackexchange.com/questions/35422/partition-numbering-and-pdf-bookmark-generation/35430#35430
\usepackage[bookmarksnumbered]{hyperref}

%\hypersetup{hidelinks,backref=true,pagebackref=true,hyperindex=true,hypertexnames=false,colorlinks=false,breaklinks=true,bookmarks=true,bookmarksopen=false,pdftitle={Title},pdfauthor={Author}}



\usepackage[capitalize]{cleveref}
%\usepackage{cleveref}
\Crefname{equation}{Equation}{Equations}
\crefname{equation}{Equation}{Equations}
\Crefname{section}{Section}{Sections}
\crefname{section}{Section}{Sections}
\Crefname{chapter}{Chapter}{Chapters}
\crefname{chapter}{Chapter}{Chapters}
\Crefname{figure}{Figure}{Figures}
\crefname{figure}{Figure}{Figures}
\Crefname{appsec}{Appendix}{Appendices}
\crefname{appsec}{Appendix}{Appendices}
%\usepackage[noabbrev,capitalize,nameinlink]{cleveref}


%https://robjhyndman.com/hyndsight/squeezing-space-with-latex/
%\usepackage{fontspec}
%setmonofont{DejaVu Sans Mono}[Scale=MatchLowercase]
%\setmainfont{DejaVu Sans}
%There is no ∇ (U+2207) in font ec-lmr10!

%http://www.gang.umass.edu/~franz/latexmanual.pdf


%https://image-color.com/color-picker#DA4F4F



\definecolor{cyan}{cmyk}{1,0,0,0.4}
\definecolor{magenta}{cmyk}{0,1,0,0.15}
\definecolor{yellow}{cmyk}{0,0,1,0}
\definecolor{black}{cmyk}{0,0,0,1}
\definecolor{orange}{cmyk}{0,0.5,1,0}
\definecolor{red}{cmyk}{0.00,0.92,0.92,0.06}
\definecolor{blue}{cmyk}{0.92,0.92,0.00,0.06}
\definecolor{green}{cmyk}{0.88,0.00,0.78,0.03}

\hypersetup{
    colorlinks,
    citecolor=magenta,
    linkcolor=magenta,
    urlcolor=cyan,
}

\usepackage{eqnalign}
\usepackage{version}

% Provide toggle to enable if..else conditions
\usepackage{etoolbox}

